A Deeper Look into Hybrid Images

$Hybrid$ $images$ was first introduced by Olivia et al., that produced static images with two interpretations such that the images changes as a function of viewing distance. Hybrid images are built by studying human processing of multiscale images and are motivated by masking studies in visual perception. The first introduction of hybrid images showed that two images can be blend together with a high pass filter and a low pass filter in such a way that when the blended image is viewed from a distance, the high pass filter fades away and the low pass filter becomes prominent. Our main aim here is to study and review the original paper by changing and tweaking certain parameters to see how they affect the quality of the blended image produced. We have used exhaustively different set of images and filters to see how they function and whether this can be used in a real time system or not.

==> buetcseugthesisalgorithms.tex <==
\chapter{Algorithms}\label{ch:algorithms}

\section{Sample Algorithm}
In Algorithm~\ref{alg1} we show how to calcute $y=x^n$.

\begin{algorithm}
  \caption{Calculate $y = x^n$}
  \label{alg1}
  \begin{algorithmic}
    \input{algorithms/yxn.alg}
  \end{algorithmic}
\end{algorithm}

\endinput


==> buetcseugthesischapterwithmathintitle.tex <==
\chapter{$k$-safe Labeling of Petersen Graph}\label{safeklabelingpetersen}

In 1898, Petersen produced a trivalent graph with no leaves, now
called the Petersen graph~\cite{holton1993petersen}.  In this chapter
we study $k$-safe labeling for the Petersen graph. We also give upper
bound for the span of the Petersen graph. We provide necessary proof
for the upper bound.

\endinput



==> buetcseugthesisciteexamples.tex <==
\chapter{Citation Examples}\label{ch:citations}

In this chapter we show how we can cite the references.


\section{See the Citations}
\label{sec:cite}

As discussed by authors
in~\cite{akbar2006solving,karim2015comograd,alam2012diversity} we can
further show how this affects
us. Moreover~\cite{kaykobad1987nonnegative,kaykobad1985positive,kaykobad19983,MCNC,guo2001floorplanning,holland1975as,aickelin2005artificial,al2010artificial}
can be examples for the previous works. Among
these~\cite{aickelin2005artificial,faruque2016modelling,durocher2015graphs,rahman2016absent,hashem2013countering,farhad2016mapping,malek2016balanced}
are the prominent ones. Also you can take a look
at~\cite{bashir2016learning,uddin2014citizen,kamal2016boosting,haque2013constructing,mukta2016identifying,ali2016spatial,islam2009new,al2010stable}.


\endinput





==> buetcseugthesisindexcreation.tex <==
\chapter{Index Creation}
\section{BUET}
Bangladesh University of Engineering and Technology, abbreviated as
BUET\index{BUET}, is one of the most prestigious institutions for
higher studies in the country. About 5500 students are pursuing
undergraduate\index{BUET!undergraduate} and
postgraduate\index{BUET!postgraduate} studies in engineering,
architecture, planning and science in this institution. At present,
BUET has sixteen teaching departments under five faculties and it has
three institutes. Every year the intake of undergraduate students is
around 900, while the intake of graduate students in Master's and PhD
programs is around 1000. A total of about five hundred teachers are
teaching in these departments and institutes. There are additional
teaching posts like Dr.\ Rashid Professor, Professor Emeritus and
Supernumerary Professors.
 
\section{Campus}
The BUET campus is in the heart of Dhaka\index{Dhaka} --- the capital
city of Bangladesh. It has a compact campus with halls of residence
within walking distances of the academic buildings. The physical
expansion of the University over the last three decades has been
impressive with construction of new academic buildings,
auditorium\index{BUET!auditorium} complex, halls of residence, etc.
 
\section{History}\index{BUET!History}
BUET is the oldest institution for the study of Engineering and
Architecture in Bangladesh. The history of this institution dates back
to the days of Dhaka Survey School which was established at
Nalgola\index{Nalgola}, in Old Dhaka in 1876 to train Surveyors for
the then Government of Bengal of British India. As the years passed,
the Survey School became the Ahsanullah School of
Engineering\index{Ahsanullah School of Engineering} offering
three-year diploma courses in Civil, Electrical and Mechanical
Engineering. In recognition of the generous financial contribution
from the then Nawab of Dhaka, it was named after his father Khawja
Ahsanullah. It moved to its present premises in 1912. In 1947, the
School was upgraded to Ahsanullah Engineering College as a Faculty of
Engineering under the University of Dhaka, offering four-year
bachelor’s courses in Civil, Electrical, Mechanical, Chemical and
Metallurgical Engineering. In order to create facilities for
postgraduate studies and research, Ahsanullah Engineering College was
upgraded to the status of a University in 1962 and was named East
Pakistan University of Engineering and Technology. After the War of
Liberation in 1971\index{1971|see {War of Liberation}}\index{War of
  Liberation}, Bangladesh became an independent state and the
university was renamed as the Bangladesh University of Engineering and
Technology.
 
\section{Students}
Till today, it has produced around 25,000 graduates in different
branches of engineering and architecture, and has established a good
reputation all over the world for the quality of its graduates, many
of whom have excelled in their profession in different parts of the
globe. It was able to attract students from countries like
India\index{India}, Nepal\index{Nepal}, Iran\index{Iran},
Jordan\index{Jordan}, Malaysia\index{Malaysia}, Sri Lanka\index{Sri
  Lanka}, Pakistan\index{Pakistan} and Palestine\index{Palestine}.
 
\section{Departments}
Both Undergraduate and Postgraduate studies and research are now among
the primary functions of the University. Eleven departments under five
faculties offer Bachelor Degrees, while most of the departments and
institutes offer Master's Degrees and some of the departments have
Ph.D. programs. In addition to its own research programs, the
university undertakes research programs sponsored by outside
organizations like European Union, UNO,
Commonwealth\index{Commonwealth}, UGC\index{UGC}, etc. The expertise
of the University teachers and the laboratory facilities of the
University are also utilized to solve problems and to provide
up-to-date engineering and technological knowledge to the various
organizations of the country.


\endinput

==> inputs/abstract.tex <==
% Write theis abstract here as LaTeX text

$Hybrid$ $images$ was first introduced by Olivia et al., that produced static images with two interpretations such that the images changes as a function of viewing distance. Hybrid images are built by studying human processing of multiscale images and are motivated by masking studies in visual perception. The first introduction of hybrid images showed that two images can be blend together with a high pass filter and a low pass filter in such a way that when the blended image is viewed from a distance, the high pass filter fades away and the low pass filter becomes prominent. Our main aim here is to study and review the original paper by changing and tweaking certain parameters to see how they affect the quality of the blended image produced. We have used exhaustively different set of images and filters to see how they function and whether this can be used in a real time system or not. 



\endinput

==> inputs/acknowledgement.tex <==
% Write the acknowledgement text here as LaTeX text

It is ritual that scholars express their gratitude to their supervisors. This
acknowledgement is very special to me to express my deepest sense of gratitude and
pay respect to my supervisor, Tamal Maharaj, Department of
Computer Science, for his constant encouragement, guidance, supervision, and support
throughout the completion of my project. His close scrutiny, constructive criticism, and
intellectual insight have immensely helped me in every stage of my work.
\\

I’m grateful to my father, Dr. Jadab Kumar Pal, Deputy Chief Executive, Indian
Statistical Institute, Kolkata for constantly motivating and supporting me to develop
this documentation along with the application. Finally, I acknowledge the help received from all my friends and well-wishers whose constant motivation has promoted the completion of this project.


\endinput
